Retractions in Intersection Types

This paper deals with retraction - intended as isomorphic embedding - in intersection types building left and right inverses as terms of a lambda calculus with a bottom constant. The main result is a necessary and sufficient condition two strict intersection types must satisfy in order to assure the existence of two terms showing the first type to be a retract of the second one. Moreover, the characterisation of retraction in the standard intersection types is discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{N. Kobayashi (Ed.): Eighth Workshop\\
on Intersection Types and Related Systems (ITRS 2016).\\
EPTCS 242, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.242.5}{10.4204/EPTCS.242.5}}

